Architectural Co-LOD Generation

Managing the level-of-detail (LOD) in architectural models is crucial yet challenging, particularly for effective representation and visualization of buildings. Traditional approaches often fail to deliver controllable detail alongside semantic consistency, especially when dealing with noisy and inconsistent inputs. We address these limitations with \emph{Co-LOD}, a new approach specifically designed for effective LOD management in architectural modeling. Co-LOD employs shape co-analysis to standardize geometric structures across multiple buildings, facilitating the progressive and consistent generation of LODs. This method allows for precise detailing in both individual models and model collections, ensuring semantic integrity. Extensive experiments demonstrate that Co-LOD effectively applies accurate LOD across a variety of architectural inputs, consistently delivering superior detail and quality in LOD representations.

==> tables/Datasets.tex <==
\begin{table*}[]
    \caption{3D Building model datasets post-2020. UAV Pt and ALS denote Unmanned Aerial Vehicle Photography and Aerial Laser Scanning, respectively. PC stands for Point Cloud. 'With Normal' indicates whether point clouds or meshes include normal information. 'Internal Face' denotes whether models contain internal faces. 'Utilization' signifies whether our method has been tested on the respective dataset.}
    \label{table:Dataset}
    \begin{tabular}{c|c|c|c|c|c|c}
    dataset          & Acquisition     & Data-type & Points/Triangles & With Normal & Internal Face & Utilization \\ \hline
    Toronto-3D~\cite{tan2020toronto3d} & ALS             & PC        & 78.3M            & $\checkmark$           & $\times$             & $\checkmark$           \\
    SensatUrban~\cite{hu2022sensaturban}      & UAV Pt        & PC        & 2847M            & $\times$           & $\times$             & $\times$           \\
    Campus3D~\cite{li2020campus3d}         & UAV Pt        & PC        & 937.1M           & $\times$           & $\times$             & $\times$           \\
    SUM~\cite{sum2021}              & Airplane Camera & Mesh      & 19M              & $\checkmark$           & $\times$             & $\checkmark$           \\
    Swiss3DCities~\cite{Swiss3DCities}    & UAV Pt        & PC        & 226M             & $\times$           & $\times$             & $\times$           \\
    STPLS3D~\cite{chen2022stpls3d}          & UAV Pt        & PC/Mesh   & 150.4M           & $\checkmark$           & $\times$             & $\checkmark$           \\
    DublinCity~\cite{zolanvari2019dublincity}       & ALS             & PC        & 260M             & $\times$           & $\times$             & $\times$           \\
    BuildingNet~\cite{BuildingNet}      & Handmade        & PC        & 200M             & $\checkmark$           & $\checkmark$             & $\times$           \\
    InstanceBuilding~\cite{instance3d} & UAV Pt        & Mesh      & 7.46M            & $\checkmark$           & $\times$             & $\checkmark$           \\
    UrbanBIS~\cite{UrbanBIS}         & UAV Pt        & PC/Mesh   & 2523.8M/284.3M   & $\checkmark$           & $\times$             & $\checkmark$          
    \end{tabular}
\end{table*}
